One-step quantum search algorithms based on smooth operators

The discovery of derivatives and integrals was a tremendous leap in scientific knowledge and completely revolutionized many fields, including mathematics, physics, and engineering. The existence of higher-order derivatives means better approximation and, thus, more accurate modeling of any physical phenomenon. Here we use smooth operators that are infinitely differentiable to construct two quantum search algorithms and connect these seemingly different areas. Along with smooth functions, permutation operators and the roots of unity are exploited to create quantum circuits to perform a quantum search. We validate our models through quantum simulators and test them on IBM's quantum hardware. Furthermore, we investigate the effect of noise and error propagation and demonstrate that our approach is more robust to noise compared to iterative methods like Grover's algorithm.

==> Files/test.tex <==
\begin{document}

\begin{center}
\Qcircuit @C=1em @R=.7em {
   &\lstick{\ket{0}} & \gate{U} & \gate{F} &\meter \\
   &\lstick{\ket{0}} & \gate{U} & \gate{F} &\meter \\
   &\vdots & \vdots & \vdots &\vdots\\
   &\lstick{\ket{0}} & \gate{U} & \gate{F} &\meter \\
}
\end{center}

\end{document}

